A Hierarchical Feature Engineering Framework for Automated Classification of Phonotraumatic and Non-Phonotraumatic Vocal Hyperfunction

Ambulatory neck-surface acceleration enables non-invasive monitoring of vocal hyperfunction, yet robust biomarkers for its subtypes remain limited. This study investigates the NeckVibe Challenge dataset to distinguish phonotraumatic (PVH) and non-phonotraumatic (NPVH) from healthy controls. We propose a hierarchical feature engineering framework comprising: (i) static, (ii) dynamic, (iii) ratio-based, (iv) coupling features capturing source filter interactions. While univariate statistical analysis shows strong separability for PVH but limited significance for NPVH, our machine learning pipeline, tailored for high-dimensional feature integration, identifies that coupling features are crucial for both tasks. We achieve an AUC of 0.891 for PVH and 0.728 for NPVH, suggesting that while PVH is near-linearly separable, NPVH discrimination benefits from modeling non-linear feature interactions.

==> Tables/table4.tex <==
\begin{table}[t]
\caption{Performance on the held-out test set.}
\label{tab4:results}
\centering
\footnotesize
\begin{tabular}{llcc}
\toprule
\textbf{Task} & \textbf{Target} & \textbf{AUC (ROC)} \\
\midrule
Task 1 & PVH vs. Control & \textbf{0.917} \\
Task 2 & NPVH vs. Control & 0.579 \\
\bottomrule
\vspace{-7mm}
\end{tabular}
\end{table}
